Portfolio Risk Measurement Using a Mixture Simulation Approach

Monte Carlo Approaches for calculating Value-at-Risk (VaR) are powerful tools widely used by financial risk managers across the globe. However, they are time consuming and sometimes inaccurate. In this paper, a fast and accurate Monte Carlo algorithm for calculating VaR and ES based on Gaussian Mixture Models is introduced. Gaussian Mixture Models are able to cluster input data with respect to market's conditions and therefore no correlation matrices are needed for risk computation. Sampling from each cluster with respect to their weights and then calculating the volatility-adjusted stock returns leads to possible scenarios for prices of assets. Our results on a sample of US stocks show that the Gmm-based VaR model is computationally efficient and accurate. From a managerial perspective, our model can efficiently mimic the turbulent behavior of the market. As a result, our VaR measures before, during and after crisis periods realistically reflect the highly non-normal behavior and non-linear correlation structure of the market.

==> tabs/tab_adj_port.tex <==
% Table generated by Excel2LaTeX from sheet 'adj3'
\begin{table*}[width=1.0\linewidth,cols=14,pos=t!]
  \centering
  \caption{VaR 5 \% for individual stocks}
    \begin{tabular*}{\tblwidth}{@{}LCCCCCCCCCCCCCC@{}}
    \toprule
      &   & \multicolumn{3}{c}{$N_c = 3$} & \multicolumn{3}{c}{$N_c = 4$} & \multicolumn{3}{c}{$N_c = 5$} & \multicolumn{3}{c}{$N_c = 6$} \\
      &   & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} \\
    \midrule
    \multirow{2}[4]{*}{Portfolio VaR} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
    \midrule
    \multirow{2}[4]{*}{Portfolio ES} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
    \bottomrule
    \end{tabular*}%
  \label{tab_adj_port}%
\end{table*}%


==> tabs/tab_ajd_stocks.tex <==
% Table generated by Excel2LaTeX from sheet 'adj3'
\begin{table*}[width=1.0\linewidth,cols=14,pos=t!]
  \centering
  \caption{VaR 5 \% for individual stocks}
    \begin{tabular*}{\tblwidth}{@{}LCCCCCCCCCCCCCC@{}}
    \toprule
      &   & \multicolumn{3}{c}{$N_c = 3$} & \multicolumn{3}{c}{$N_c = 4$} & \multicolumn{3}{c}{$N_c = 5$} & \multicolumn{3}{c}{$N_c = 6$} \\
      &   & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} & \multicolumn{1}{c}{70} & \multicolumn{1}{c}{80} & \multicolumn{1}{c}{90} \\
    \midrule
    \multirow{2}[4]{*}{S\&P500} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{MMM} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AXP} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AMD} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AIG} & 1 & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AFL} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{ABT} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{MSFTF} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AAPL} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{AMZN} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{BAC} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{JPM} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{JNJ} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} & \cellcolor[rgb]{ .647,  0,  .129} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{XOM} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}    \multirow{2}[4]{*}{MA} & 1 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
\cmidrule{3-14}      & 5 & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} & \cellcolor[rgb]{ .573,  .816,  .314} \\
    \bottomrule
    \end{tabular*}%
  \label{tab_sssss}%
\end{table*}%

